Interpretable Biomanufacturing Process Risk and Sensitivity Analyses for Quality-by-Design and Stability Control

While biomanufacturing plays a significant role in supporting the economy and ensuring public health, it faces critical challenges, including complexity, high variability, lengthy lead time, and very limited process data, especially for personalized new cell and gene biotherapeutics. Driven by these challenges, we propose an interpretable semantic bioprocess probabilistic knowledge graph and develop a game theory based risk and sensitivity analyses for production process to facilitate quality-by-design and stability control. Specifically, by exploring the causal relationships and interactions of critical process parameters and quality attributes (CPPs/CQAs), we create a Bayesian network based probabilistic knowledge graph characterizing the complex causal interdependencies of all factors. Then, we introduce a Shapley value based sensitivity analysis, which can correctly quantify the variation contribution from each input factor on the outputs (i.e., productivity, product quality). Since the bioprocess model coefficients are learned from limited process observations, we derive the Bayesian posterior distribution to quantify model uncertainty and further develop the Shapley value based sensitivity analysis to evaluate the impact of estimation uncertainty from each set of model coefficients. Therefore, the proposed bioprocess risk and sensitivity analyses can identify the bottlenecks, guide the reliable process specifications and the most "informative" data collection, and improve production stability.

==> latexmacro.tex <==

%% LaTeX2e file `latexmacro.tex'
%% generated by the `filecontents' environment
%% from source `Gkmn51' on 2001/03/06.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  This macro contains definitions of new \LaTeX commands  %%
%%  that are frequently used by Barry L. Nelson.  This is   %%
%%  a new release of the 'latexmacro.tex' file that I have  %%
%%  distributed for some time.  This release                %%
%%  is designed to be compatible with previous releases,    %%
%%  except for eliminating the \smallheads command.         %%
%%                                                          %%
%%  This releases fixes a few bugs (please report any you   %%
%%  find to nelsonb@random.eng.ohio-state.edu), includes    %%
%%  more documentation, and completes the definitions of    %%
%%  bold-face mathematics characters.                       %%
%%                                                          %%
%%  release 2.01   1/2/92                                   %%
%%  unreleased update 6/9/92  6/22/92 1/19/93 2/3/93        %%
%%                    6/2/93  8/15/93 11/11/93 11/23/93     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% USING THE MACRO:
%% If you name this file latexmacro.tex, then use the following
%% statement just after the \documentstyle{} command:
%%
%%    \input [path] latexmacro
%%
%% LINE SPACING:
%% Define single, one and a half, and double space commands; these
%% may be used anywhere after \begin{document}
%%
\def\double{\par\baselineskip=24pt}
\def\single{\par\baselineskip=12pt}
\def\oneandahalf{\par\baselineskip=18pt}
%%
%% TEXT DIMENSIONS
%% Define text widths \standard, \proceedings and \myletter.
%% \proceedings prints a single, narrow column near the edge of the page.
%% Use these before \begin{document} command.
%%
\def\standard{\oddsidemargin=0in
              \evensidemargin=0in
              \topmargin =-.5in
              \textheight=8.5in
              \textwidth=6.5in}
\def\proceedings{\oddsidemargin=-.5in
                 \evensidemargin=-.5in
                 \textwidth=4.56in
                 \parindent=0.3in
                 \topmargin=-1in
                 \textheight=10in
                 \pagestyle{empty}}
\def\myletter{\oddsidemargin=.3in
                 \evensidemargin=.3in
                 \baselineskip=16pt
                 \textwidth=5.5in
                 \pagestyle{empty}}
%%
%% Define command to pull in letterhead file.
%% This command is specific to VAX/VMS and Arbortext dvips program.
%% Insert your own path.
%%
\def\letterhead{\special{ps: plotfile [is.nelson.com]letterhead.tex 
local}}
%%
%%
%% LISTS:
%% Define \plainlist environment
%%
\newenvironment{plainlist}
{\begin{list}%
{}{\setlength{\leftmargin}{\rightmargin}\setlength{\labelwidth}{0in}}}%
{\end{list}}
%%
%% Define \hangref environment for hanging indentation
%%
\newenvironment{hangref}{\begin{list}{}{\setlength{\itemsep}{0pt}%
\setlength{\parsep}{0pt}\setlength{\leftmargin}{+\parindent}%
\setlength{\itemindent}{-\parindent}}}{\end{list}}
%%
%%
%%
%%
%% MATHEMATICS:
%%Special math symbols
%%
%% operators
\def\E{{\rm E}}
\def\Var{{\rm Var}}
\def\Cov{{\rm Cov}}
\def\Corr{{\rm Corr}}
\def\Bias{{\rm Bias}}
\def\MSE{{\rm MSE}}
\def\CP{{\rm CP}}
\def\trace{{\rm trace}}
\def\tr{{\rm tr}}
%%
%% bold face roman
\def\bA{{\bf A}}
\def\ba{{\bf a}}
\def\bB{{\bf B}}
\def\bb{{\bf b}}
\def\bC{{\bf C}}
\def\bc{{\bf c}}
\def\bD{{\bf D}}
\def\bd{{\bf d}}
\def\bE{{\bf E}}
\def\be{{\bf e}}
\def\bF{{\bf F}}
\def\boldf{{\bf f}}
\def\bG{{\bf G}}
\def\bg{{\bf g}}
\def\bH{{\bf H}}
\def\bh{{\bf h}}
\def\bi{{\bf i}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bj{{\bf j}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
\def\bL{{\bf L}}
\def\bl{{\bf l}}
\def\bM{{\bf M}}
\def\bm{{\bf m}}
\def\bN{{\bf N}}
\def\bn{{\bf n}}
\def\bO{{\bf O}}
\def\bo{{\bf o}}
\def\bP{{\bf P}}
\def\bp{{\bf p}}
\def\bQ{{\bf Q}}
\def\bq{{\bf q}}
\def\bR{{\bf R}}
\def\br{{\bf r}}
\def\bS{{\bf S}}
\def\bs{{\bf s}}
\def\bT{{\bf T}}
\def\bt{{\bf t}}
\def\bU{{\bf U}}
\def\bu{{\bf u}}
\def\bV{{\bf V}}
\def\bv{{\bf v}}
\def\bW{{\bf W}}
\def\bw{{\bf w}}
\def\bX{{\bf X}}
\def\bx{{\bf x}}
\def\bY{{\bf Y}}
\def\by{{\bf y}}
\def\bZ{{\bf Z}}
\def\bz{{\bf z}}
%%
%% bold face Greek (incomplete)
\def\balpha{\mbox{\boldmath $\alpha$}}
\def\bbeta{\mbox{\boldmath $\beta$}}
\def\bepsilon{\mbox{\boldmath $\epsilon$}}
\def\bvarepsilon{\mbox{\boldmath $\varepsilon$}}
\def\bDelta{{\bf \Delta}}
\def\bdelta{\mbox{\boldmath $\delta$}}
\def\boldeta{\mbox{\boldmath $\eta$}}
\def\bGamma{{\bf \Gamma}}
\def\bgamma{\mbox{\boldmath $\gamma$}}
\def\bLambda{{\bf \Lambda}}
\def\blambda{\mbox{\boldmath $\lambda$}}
\def\bmu{\mbox{\boldmath $\mu$}}
\def\bOmega{{\bf \Omega}}
\def\bpi{\mbox{\boldmath $\pi$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bPsi{{\bf \Psi}}
\def\bpsi{\mbox{\boldmath $\psi$}}
\def\bSigma{{\bf \Sigma}}
\def\bsigma{\mbox{\boldmath $\sigma$}}
\def\bTheta{{\bf \Theta}}
\def\btheta{\mbox{\boldmath $\theta$}}
\def\bXi{{\bf \Xi}}
\def\bxi{\mbox{\boldmath $\xi$}}
%%
%% misc. Greek with hats
\def\betahat{\hat \beta}
\def\bbetahat{\hat{\mbox{\boldmath $\beta$}}}
\def\bdeltahat{\hat{\mbox{\boldmath $\delta$}}}
\def\etahat{\hat{\eta}}
\def\epsilonhat{\hat{\epsilon}}
\def\bepsilonhat{\hat{\mbox{\boldmath $\epsilon$}}}
\def\bgammahat{\hat{\mbox{\boldmath $\gamma$}}}
\def\bmuhat{\hat{\mbox{\boldmath $\mu$}}}
\def\thetahat{\hat \theta}
%%
%% caligraphy letters
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cI{{\cal I}}
\def\cM{{\cal M}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cY{{\cal Y}}
%%
%% tt letters
\def\tS{{\tt S}}
\def\tC{{\tt C}}
\def\tI{{\tt I}}
\def\tT{{\tt T}}
%%
%% vec notation
\def\vp{\vec{p}}
\def\bvP{\vec{{\bf P}}}
%%
%% bold face numbers
\def\b1{{\bf 1}}
\def\bzero{{\bf 0}}
%%
%% \blot gives a square at end of formulas and proofs
%% (thanks to Marc Posner)
\def\blot{\quad {$\vcenter{\vbox{\hrule height.4pt
             \hbox{\vrule width.4pt height.9ex \kern.9ex \vrule 
width.4pt}
             \hrule height.4pt}}$}}
%%
%% End of latexmacro
